Environmental Impact of Hardware Usage and Replacement Practices in Local AI Training

Improving the energy efficiency of AI workloads through next-generation hardware can reduce their environmental footprint, but producing this hardware also has significant impacts, and efficiency improvements can lead to rebound effects. Understanding the impacts of hardware upgrades and adopting good practices is particularly important for small-scale local AI infrastructure, such as that used by research laboratories and small companies. In this work, we investigate how hardware upgrades and usage patterns affect the environmental footprint of AI training at a local scale. Using direct power measurements, we evaluate the energy efficiency of a representative computer vision workload, training a Vision Transformer across PyTorch versions, performance optimization techniques, and hardware setups spanning five NVIDIA GPU generations and multiple server configurations. We then assess and discuss the operational and embodied impacts of concrete upgrade and workload evolution scenarios over a six-year period, considering three locations and environmental impact categories: climate change, water use, and abiotic depletion. Our study shows that the environmental benefits of hardware upgrades depend strongly on usage and workload evolution patterns, and the location and environmental category considered. We also find that the impact of good practices can be significant compared to hardware upgrades: software updates alone can reduce impacts or enable workload growth; turning off idle servers can lead to considerable impact reduction; and upgrading components other than GPUs can exacerbate impacts for compute-bound workloads. Importantly, our study also points out the potentially dramatic impact of increasing workloads to match hardware capacity. We hope that our analysis, based on the technical evolution of the last six years, will provide insights to guide future decisions and policy design.

==> tikz/common_styles/all_hardware_common.tex <==

\input{data/all_hardware_data}

\def\effYmax{1.7}
\def\thrYmaxSmall{650}      %
\def\thrYmaxLarge{1200}     %

\def\panelcoords#1{symbolic x coords={#1}, xtick={#1}}

\pgfplotsset{
    hardware panel/.style={
        common barplot,
        ybar=-3mm,
        height=1.8cm,
    },
    reference bar/.style={fill=gray!80},
}

\pgfplotsset{
    gpu panel/.style={
        name=plot1,
        hardware panel,
        width=0.37\textwidth,
        title=\textcolor{ForestGreen!60}{\textbf{GPU}},
        \panelcoords{titanx_16, titanxp_32, p5000_16, 1080ti_32, 2080ti_64, 2070super_64, a6000_512, a5000_256},
        xticklabels={
            Titan X \textcolor{gray}{\footnotesize(2015)},
            Titan X (Pascal) \textcolor{gray}{\footnotesize(2016)},
            P5000 \textcolor{gray}{\footnotesize(2016)},
            1080 Ti \textcolor{gray}{\footnotesize(2017)},
            2080 Ti \textcolor{gray}{\footnotesize(2018)},
            2070 SUPER \textcolor{gray}{\footnotesize(2019)},
            \textbf{A6000 \textcolor{gray}{\footnotesize(2020)}},
            5000 Ada \textcolor{gray}{\footnotesize(2023)}
        },
    },
    two gpu panel/.style={
        at={(plot1.south west)},
        anchor=north west,
        yshift=-2.2cm,
        name=plot2,
        hardware panel,
        width=0.1\textwidth,
        title=\textcolor{red!60}{\textbf{Two GPU}},
        \panelcoords{no_nvlink, nvlink},
        xticklabels={No NVLink, With NVLink},
    },
    ram panel/.style={
        at={(plot2.north east)},
        anchor=north west,
        xshift=5pt,
        name=plot3,
        hardware panel,
        width=0.13\textwidth,
        yticklabel=\empty,
        title=\textcolor{orange!60}{\textbf{RAM}},
        \panelcoords{32gb, 48gb, 64gb},
        xticklabels={
            32 GB \textcolor{gray}{\footnotesize($70\%$ util.)},
            48 GB \textcolor{gray}{\footnotesize($45\%$ util.)},
            \textbf{64 GB \textcolor{gray}{\footnotesize($35\%$ util.)}}
        },
    },
    disk panel/.style={
        at={(plot3.north east)},
        anchor=north west,
        xshift=5pt,
        name=plot4,
        hardware panel,
        width=0.17\textwidth,
        yticklabel=\empty,
        title=\textcolor{violet!60}{\textbf{Disk}},
        \panelcoords{hdd, hdd_wds, sata_ssd, nvme_ssd},
        xticklabels={HDD, HDD+WebDataset, SATA SSD, \textbf{NVMe SSD}},
    },
    cpu panel/.style={
        at={(plot4.north east)},
        anchor=north west,
        xshift=5pt,
        name=plot5,
        hardware panel,
        width=0.3\textwidth,
        yticklabel=\empty,
        title=\textcolor{magenta!60}{\textbf{CPU}},
        \panelcoords{zalman, dellhp, hephaistos, ares, methis, moravia, hermes},
        xticklabels={
            Core i7-5820K \textcolor{gray}{\footnotesize(2014)},
            Xeon E5-2609 v4 \textcolor{gray}{\footnotesize(2016)},
            Core i7-6900K \textcolor{gray}{\footnotesize(2016)},
            Core i7-7820X \textcolor{gray}{\footnotesize(2017)},
            Core i9-9900X \textcolor{gray}{\footnotesize(2018)},
            \textbf{Xeon Silver 4208 \textcolor{gray}{\footnotesize(2019)}},
            Xeon Silver 4210R \textcolor{gray}{\footnotesize(2020)}
        },
    },
    pcie panel/.style={
        at={(plot5.north east)},
        anchor=south east,
        yshift=2.2cm,
        name=plot6,
        hardware panel,
        width=0.3\textwidth,
        yticklabel=\empty,
        title=\textcolor{blue!60}{\textbf{PCIe Bandwidth}},
        \panelcoords{x1gen1, x1gen2, x1gen3, x8gen1, x16gen1, x16gen2, x16gen3},
        xticklabels={250 MB/s, 500 MB/s, 1 GB/s, 2 GB/s, 4 GB/s, 8 GB/s, \textbf{16 GB/s}},
    },
}


==> tikz/common_styles/carbon_all_scenarios_common.tex <==

\pgfplotsset{
    carbon barplot/.style={
        common barplot,
        width=0.15\textwidth,
        height=1.8cm,
        enlarge x limits={abs=10pt},
        title style={yshift=-5pt},
        ybar=0,
        bar width=1.5mm,
        legend columns=3,
        yticklabel style={xshift=10},
        legend style={
            at={(0.64,0.83)},
            anchor=east,
            nodes={scale=0.9},
        },
        symbolic x coords={constant, exponential, adjusted},
        xtick={constant, exponential, adjusted},
        xticklabels={Constant, Exponential, Adjusted},
    },
    infeasible scenario cross/.style={
        only marks,
        mark=x,
        mark size=2pt,
        mark options={xshift=-1.5mm, yshift=2pt},
        draw=acces3,
        line width=0.8pt,
        forget plot,
        clip=false,
    },
}

\pgfplotsset{
    gwp panel/.style={
        carbon barplot,
        ymax=15,
    },
    water panel/.style={
        carbon barplot,
        ytick distance=1,
        ymax=4.1,
    },
    gwp sweden panel/.style={
        name=plot1,
        gwp panel,
        title={\raisebox{-2pt}{\twemoji[height=0.5cm]{flag: Sweden}}},
    },
    gwp germany panel/.style={
        at={(plot1.north east)},
        anchor=north west,
        xshift=13.5pt,
        name=plot2,
        gwp panel,
        yticklabels={},
        title={\raisebox{-2pt}{\twemoji[height=0.5cm]{flag: Germany}}},
    },
    gwp poland panel/.style={
        at={(plot2.north east)},
        anchor=north west,
        xshift=13.5pt,
        name=plot3,
        gwp panel,
        yticklabels={},
        title={\raisebox{-2pt}{\twemoji[height=0.5cm]{flag: Poland}}},
    },
    water sweden panel/.style={
        at={(plot3.north east)},
        anchor=north west,
        xshift=30pt,
        name=plot4,
        water panel,
        title={\raisebox{-2pt}{\twemoji[height=0.5cm]{flag: Sweden}}},
    },
    water poland panel/.style={
        at={(plot4.north east)},
        anchor=north west,
        xshift=13.5pt,
        name=plot6,
        water panel,
        yticklabels={},
        title={\raisebox{-2pt}{\twemoji[height=0.5cm]{flag: Poland}}},
    },
}

\def\carbonLegend{%
    \legend{\hspace{1pt}\faHistory\hspace{2pt}Keep old, \hspace{1pt}\faAngleDoubleUp\hspace{2pt}GPU once, \hspace{1pt}\faAngleDoubleUp\hspace{2pt}GPU twice}%
}

\def\gwpHeading{%
    \node[anchor=south, align=center] at ([yshift=20pt]plot2.north) {\textbf{Global Warming Potential} {\small(t CO$_2$eq)}};%
}
\def\waterHeading{%
    \node[anchor=south, align=center] at ($ (plot4.north)!0.5!(plot6.north) + (0, 20pt)$) {\textbf{Water Use} {\small(operational, m$^3$ world-eq)}};%
}

\newcommand{\trimCarbonPlotBoundingBox}{%
    \coordinate (carbonplotboundingboxsw) at (current bounding box.south west);%
    \coordinate (carbonplotboundingboxne) at (current bounding box.north east);%
    \pgfresetboundingbox
    \path[use as bounding box]
        ([yshift=14pt]carbonplotboundingboxsw)
        rectangle
        (carbonplotboundingboxne);%
}


==> tikz/common_styles/pytorch_cuda_versions_common.tex <==

\def\pytorchOptiSmallBatch#1{%
    \addplot[mark=o, ForestGreen!60, only marks, line width=1pt, mark size=2.5pt]
        table[x=release_date, y=#1, col sep=comma,
              discard if three={batch_size}{256}{tf32}{enable}{keep_small}{TRUE}]
        {data/pytorch.csv};}
\def\pytorchDefault#1{%
    \addplot[mark=triangle, only marks, color=orange!60, line width=1pt, mark size=3pt]
        table[x=release_date, y=#1, col sep=comma,
              discard if two={batch_size}{256}{tf32}{}]
        {data/pytorch.csv};}
\def\pytorchOptiLargeBatch#1{%
    \addplot[mark=o, only marks, color=ForestGreen!60, line width=1pt, mark size=3.5pt]
        table[x=release_date, y=#1, col sep=comma,
              discard if three={batch_size}{512}{tf32}{enable}{keep_small}{}]
        {data/pytorch.csv};}
\def\pytorchNoOpti#1{%
    \addplot[mark=Mercedes star, only marks, color=red!60, line width=1pt, mark size=3pt]
        table[x=release_date, y=#1, col sep=comma,
              discard if two={batch_size}{256}{tf32}{disable}]
        {data/pytorch.csv};}

\pgfplotsset{
    release year axis/.style={
        xlabel={Release date},
        height=4cm,
        width=\textwidth,
        y tick style={draw=none},
        date ZERO=2020-11-01,
        xmin=2020-08-30,
        xmax=2026-10-10,
        date coordinates in=x,
        x tick label as interval,
        xticklabels={2020, 2021, 2022, 2023, 2024, 2025, 2026},
        yticklabels=\empty,
        ymajorgrids=true,
        yminorgrids=true,
        axis lines=left,
        ylabel style={yshift=10pt},
        ymin=0,
        ymax=1.6,
        xtick={2020-01-01,2021-01-01, 2022-01-01, 2023-01-01, 2024-01-01, 2025-01-01, 2026-01-01},
    },
    release plot axis/.style={
        axis line style={draw=none},
        title style={yshift=15pt},
        width={\textwidth},
        height=4cm,
        axis x line*=top,
        xmin=2020-08-30,
        xmax=2026-10-10,
        ymin=0,
        legend cell align=left,
        xmajorgrids=true,
        xminorgrids=true,
        major grid style={color=gray!20},
        legend columns=2,
        legend style={
            /tikz/column 2/.style={
                column sep=0.3cm,
            },
            /tikz/column 4/.style={
                column sep=0.3cm,
            },
            cells={align=left},
            at={(0.955,0.49)},
            anchor=east,
            draw=gray,
            nodes={scale=0.9}
        },
        date coordinates in=x,
        ytick style={draw=none},
        xticklabel style={rotate=45, anchor=west, xshift=-2, yshift=4},
        xtick={2020-12-10, 2021-08-17, 2021-09-22, 2021-12-15, 2022-03-10, 2022-08-05, 2022-12-16, 2023-05-08, 2023-12-15, 2024-03-27, 2024-06-05, 2024-09-04, 2024-10-29, 2025-01-29, 2025-06-04, 2025-08-06, 2025-11-12, 2026-01-21, 2026-03-23, 2026-06-18},
        xticklabels={1.7.1, \raisebox{4pt}{1.8.2}, \raisebox{-4pt}{1.9.1}, 1.10.1, 1.11.0, 1.12.1, 1.13.1, 2.0.1, 2.1.2, 2.2.2, 2.3.1, 2.4.1, 2.5.1, 2.6.0, 2.7.1, 2.8.0, 2.9.1, 2.10.0, 2.11.0, 2.12.1},
    },
}


==> tikz/common_styles/pytorch_optimizations_common.tex <==

\input{data/pytorch_optimizations_data}

\def\optiYmaxEff{1.5}
\def\optiYmaxThr{650}

\pgfplotsset{
    optimization panel/.style={
        common barplot,
        enlarge x limits=0.2,
        xtick=data,
    }
}

\pgfplotsset{
    no opti panel/.style={
        name=plot1,
        optimization panel,
        width=0.05\textwidth,
        title=\textcolor{gray!80}{\textbf{None}},
        symbolic x coords={all_optimizations_off},
        xticklabels={No optimizations},
    },
    compile panel/.style={
        at={(plot1.north east)},
        anchor=north west,
        xshift=15pt,
        name=plot2,
        optimization panel,
        width=0.2\textwidth,
        title style={yshift=-2pt},
        title=\textcolor{blue!60}{\textbf{Compile}},
        yticklabel=\empty,
        symbolic x coords={compile_cudagraphs_default, compile_inductor_default, compile_inductor_reduce-overhead, compile_inductor_max-autotune},
        xticklabels={CUDA Graphs, Inductor -- Default, Inductor -- Reduce ovhd., Inductor -- Max auto.},
    },
    precision panel/.style={
        at={(plot2.north east)},
        anchor=north west,
        xshift=15pt,
        name=plot3,
        optimization panel,
        width=0.07\textwidth,
        ybar=-3mm,
        title=\textcolor{purple!60}{\textbf{Precision}},
        yticklabel=\empty,
        symbolic x coords={tf32_only, amp_only},
        xticklabels={TF32, AMP},
    },
    attention panel/.style={
        at={(plot3.north east)},
        anchor=north west,
        xshift=15pt,
        name=plot4,
        optimization panel,
        width=0.15\textwidth,
        ybar=-3mm,
        title=\textcolor{orange!60}{\textbf{Attention}},
        yticklabel=\empty,
        symbolic x coords={math_attention_amp, cudnn_attention_amp, flash_attention_amp},
        xticklabels={Math+AMP, cuDNN+AMP, Flash+AMP},
    },
    all opti panel/.style={
        at={(plot4.north east)},
        anchor=north west,
        xshift=15pt,
        name=plot5,
        optimization panel,
        width=0.05\textwidth,
        ybar=-3mm,
        title=\textcolor{ForestGreen!60}{\textbf{All}},
        yticklabel=\empty,
        symbolic x coords={all_optimizations_on},
        xticklabels={Flash+AMP+Compile},
    },
}

